Vector-Based Data Improves Left-Right Eye-Tracking Classifier Performance After a Covariate Distributional Shift

The main challenges of using electroencephalogram (EEG) signals to make eye-tracking (ET) predictions are the differences in distributional patterns between benchmark data and real-world data and the noise resulting from the unintended interference of brain signals from multiple sources. Increasing the robustness of machine learning models in predicting eye-tracking position from EEG data is therefore integral for both research and consumer use. In medical research, the usage of more complicated data collection methods to test for simpler tasks has been explored to address this very issue. In this study, we propose a fine-grain data approach for EEG-ET data collection in order to create more robust benchmarking. We train machine learning models utilizing both coarse-grain and fine-grain data and compare their accuracies when tested on data of similar/different distributional patterns in order to determine how susceptible EEG-ET benchmarks are to differences in distributional data. We apply a covariate distributional shift to test for this susceptibility. Results showed that models trained on fine-grain, vector-based data were less susceptible to distributional shifts than models trained on coarse-grain, binary-classified data.

==> data.tex <==
In our experiments, we used the EEGEyeNet dataset  \cite{kastrati2021eegeyenet}. The EEGEyeNet dataset gathers EEG and eye-tracking data from 356 (190 female and 166 male) healthy subjects of varying ages (18 - 80). Data were collected for 3 different experimental tasks according to the Declaration of Helsinki Principles. The tasks are Pro- and Antisaccade, Large Grid, and Visual Symbol Search. The recording setup was similar across all experimental tasks. EEG data were recorded using a 128-channel EEG Geodesic Hydrocel system at a sampling rate of 500 Hz. Eye position was simultaneously recorded using an infrared video-based ET EyeLink 1000 Plus also at a sampling rate of 500 Hz. Between trials, the eye-tracking device would be reset with a 9-point grid. Subjects were situated 68 cm away from a 24-inch monitor with a resolution of 800 x 600 pixels. In this study, we directly use data from the pro-antisaccade paradigm and manipulate data from the large grid paradigm to use for the analysis. 

\subsection{Pro-Antisaccade Task}
In this task, each trial starts with a central square on which the participants were asked to focus for a randomized period that doesn't exceed 3.5 seconds. Then, a dot appears horizontally to the left or the right of this central square, as shown in Figure \ref{fig:PAED}. Subjects were asked to perform a saccade towards the opposite side of the cue and then look back to the center of the screen after 1 second. Thus, gaze positions in pro-antisaccade were restricted to the horizontal axis and were binary-classified either left or right (relative to the dot at the screen's center).

\subsection{Large Grid Task}
For this task, subjects were asked to stare at a blank screen and focus on the appearing dots. A set of well-distributed dots in 25 positions would then appear one at a time for 1.5 to 1.8 seconds, as shown in Figure \ref{fig:LGPAED}. The center dot would appear three times for a total of 27 trials per block. Subjects perform 5 blocks and repeat the procedure 6 times for a total of 810 trials per subject. Thus, large grid's framework enabled fine-grain EEG-ET data collection as gaze positions were encoded using both angle and amplitude.

\begin{figure} [!t]
    \centering
    \includegraphics[scale = 0.8]{PAED.png}
    \caption{Schematic for the location of the cues on the screen in the pro-antisaccade paradigm \cite{kastrati2021eegeyenet}}
    \label{fig:PAED}
\end{figure}

\begin{figure} [!b]
    \centering
    \includegraphics[scale = 0.8]{LGED.png}
   \caption{Schematic for the location of the dots on the screen in the large grid paradigm \cite{kastrati2021eegeyenet}}
    \label{fig:LGPAED}
\end{figure}

==> intro.tex <==
\subsection{Problem Statement}
Eye-tracking (ET) is the process of predicting a subject’s point of gaze or robustly detecting the relative motion of the eye to the head \cite{klaib2021eye}. Electroencephalography (EEG) signals are brain signals that correspond to various states from the scalp surface area, encoding neurophysiological markers, and are characterized by their high temporal resolution and minimal restrictions \cite{kumar2012analysis}.

Recently, predicting eye-tracking data using EEG has received increasing interest because of the recent hardware and software technological advancements and its versatile applications in different fields \cite{sabanci2015classification,hollenstein2018zuco,kastrati2021eegeyenet}. For instance, EEG-ET data can be used to identify shopping motives relatively early in the search process \cite{pfeiffer2020eye}, to detect workload strain in truck drivers \cite{lobo2016cognitive}, and to assess the diagnosis of many neurological diseases such as Autism Spectrum Disorder and Alzheimer's \cite{thapaliya2018evaluating,sotoodeh2021preserved,kang2020identification}. 

With the broad array of EEG-ET data applications, accuracy and efficiency are of utmost importance. The collection of both EEG and ET data, however, involves challenges such as finding invariant representation of inter-and intra-subject differences as well as noise resulting from the unintended interference of brain signals from multiple sources \cite{wu2022learning}. Increasing the robustness of machine learning models in making accurate eye-tracking predictions from EEG data is therefore integral for both research and consumer use.


\subsection{Literature Review}
EEG is a type of highly individualized time-series data \cite{qu2018personalized,qu2018eeg,qu2020identifying,roy2019deep}. Machine Learning approaches perform adequately on computer vision, bioinfomatics, medical image analysis and usually have potential in EEG analysis as well \cite{qian2021two,qian2020multi,gu2020multi,xu2020multi}. Machine Learning and Deep Learning methods have been implemented in EEG classification research with promising results \cite{lotte2018review,qu2020multi,qu2020using,craik2019deep}. Recent works in this area have focused on determining what machine learning models are more capable of predicting eye position from EEG signals. In that pursuit, \cite{lotte2018review} has shown that Riemannian geometry and tensor-based classification methods have reached state-of-the-art performances in multiple EEG-based machine learning applications. Previous work has also been done in collecting large datasets that combine EEG and ET data. A good example is the multi-modal neurophysiological dataset collected by \cite{langer2017resource} and EEGEyeNet \cite{kastrati2021eegeyenet}. Finally, other work has been done to eliminate the noise associated with EEG data collection automatically, such as \cite{plochl2012combining,oikonomou2020machine}. Also, \cite{roy2019machine} showed the potential of using machine learning for noise elimination. Soon after, Zhang et al. collected EEGdenoiseNet, a dataset suitable to train machine learning models in noise elimination \cite{zhang2021eegdenoisenet}. These benchmarks include ocular artifacts; thus, they apply to EEG data collected simultaneously with eye-tracking data. 

While much work has been done to improve the accuracy of ET-based EEG applications, there is a lack of previous work that focuses on examining the effects of data collection methods on eye position prediction accuracies. In particular, we are interested in comparing coarse-grain and fine-grain data collection techniques for simultaneously collecting EEG and eye-tracking data. In other fields of medical research, fine-grain data collection methods have been explored with great success \cite{higginson2000ecological,plancher2012using}. That is using more complicated data collection methods to test for less complicated tasks. Often, systems developed in "lab conditions" only work in controlled environments, causing difficulties when utilized in uncontrolled conditions \cite{wilson1993,marcotte2010neuropsychology}. With consumer EEG-ET applications becoming increasingly prevalent, the importance of assessing whether finer-grain data collection methods improve upon the accuracy and robustness of EEG-ET machine learning classifiers is magnified. To narrow down this assessment, this study focuses on the effects of training machine learning models on fine- versus coarse-grain EEG data in predicting the binary direction (left or right) of eye-tracking position. 

\subsection{Purpose of Study}
Previously, benchmarks for left-right eye-tracking predictions were established utilizing data from binary-classified data collection methods \cite{kastrati2021eegeyenet}. In this study, we train machine learning models for left-right eye-tracking classification using data from a vector-based collection framework. We then compare the results to the models trained by Kastrati et al. and determine whether finer-grain data is beneficial to the robustness of EEG-ET machine learning models. Robustness is determined by the accuracy after a covariate distributional shift. This attempts to mimic realistic data with varying distributional patterns.
The purpose of this study is to verify whether machine learning models trained using vector-based, fine-grain eye-tracking data obtain higher accuracies in left-right gaze classification than models trained using binary-based, coarse-grain eye-tracking data after a covariate shift is applied. 
